Vul-RAG: Enhancing LLM-based Vulnerability Detection via Knowledge-level RAG

Although LLMs have shown promising potential in vulnerability detection, this study reveals their limitations in distinguishing between vulnerable and similar-but-benign patched code (only 0.06 - 0.14 accuracy). It shows that LLMs struggle to capture the root causes of vulnerabilities during vulnerability detection. To address this challenge, we propose enhancing LLMs with multi-dimensional vulnerability knowledge distilled from historical vulnerabilities and fixes. We design a novel knowledge-level Retrieval-Augmented Generation framework Vul-RAG, which improves LLMs with an accuracy increase of 16% - 24% in identifying vulnerable and patched code. Additionally, vulnerability knowledge generated by Vul-RAG can further (1) serve as high-quality explanations to improve manual detection accuracy (from 60% to 77%), and (2) detect 10 previously-unknown bugs in the recent Linux kernel release with 6 assigned CVEs.

==> picture/detection.tex <==
\begin{figure}[htb]
	\centering
        %\vspace{-3mm}
	\includegraphics[width=0.9\linewidth]{pictures/detection.pdf}
	\caption{Example of Knowledge-driven RAG-based Vulnerability Knowledge Detection}
	\label{fig:detection}
    %\vspace{-2mm}
        
\end{figure}

==> picture/rag.tex <==
\begin{figure}[htb]
	\centering
        %\vspace{-3mm}
	\includegraphics[width=0.8\linewidth]{pictures/rag.pdf}
	\caption{The LLM-based RAG Architecture}
	\label{fig:rag}
    %\vspace{-2mm}
        
\end{figure}

==> section/background.tex <==
\section{Background}
\subsection{CVE and CWE}
% \subsubsection{Software Vulnerability}
% \lmw{add an overview sentence}
Existing vulnerability classification systems, such as Common Vulnerabilities and Exposures (CVE)~\cite{cve} and Common Weakness Enumeration (CWE)~\cite{cwe}, provide a comprehensive taxonomy of categorizing and managing vulnerabilities. 
{CVE} is a publicly disclosed list of common security vulnerabilities. Each vulnerability is assigned a unique identifier (CVE ID). A single CVE ID may be associated with multiple distinct code snippets. 

{CWE} is a publicly accessible classification system of common software and hardware security vulnerabilities. Each weakness type within this enumeration is assigned a unique identifier (CWE ID). While CWE provides a broad classification of vulnerability types, the specific code behaviors leading to a vulnerability under a given CWE category may vary widely. For example, CWE-416 (Use After Free)~\cite{cwe416} signifies the issue of referencing memory after it has been freed. The root cause of this vulnerability might stem from improper synchronization under race conditions (\eg{} CVE-2023-30772~\cite{cve-2023-30772}), or errors in reference counting leading to premature object destruction (\eg{} CVE-2023-3609~\cite{cve-2023-3609}). 



\subsection{LLM-based Vulnerability Detection}



This category leverages large language models (LLMs) for vulnerability detection via prompt engineering or fine-tuning~\cite{DBLP:journals/corr/abs-2308-12697, DBLP:conf/icse/YangGMH24, DBLP:journals/corr/abs-2401-17010}. The former leverages different prompting strategies, \eg{} Chain-of-Thought (CoT)~\cite{wei2023chainofthought, zhang2022automatic} and few-shot learning~\cite{ahmed2022few, brown2020language, mao2024effectivelydetectingexplainingvulnerabilities} for more accurate LLM-based vulnerability detection, without modifying the original LLM parameters; the latter updates LLM parameters by trained on vulnerability detection datasets, to learn the features of vulnerable code. 

\subsection{Retrieval-Augmented Generation}
Retrieval-Augmented Generation (RAG) is a general paradigm that enhances LLMs by including relevant information retrieved from external databases into the input~\cite{gao2024retrievalaugmented}. RAG typically consists of three phases: indexing, retrieval, and generation. First, the indexing phase constructs external databases and their retrieval index from external data sources;  Second, given a user query, the retrieval system then utilizes these indexes to fetch the relevant document chunks as context. Third, the retrieved context is then integrated into the input prompt for LLMs, and LLMs then generate the final output based on the augmented inputs. RAG has been widely used in various domains~\cite{DBLP:conf/nips/LewisPPPKGKLYR020, DBLP:conf/emnlp/ShiW0DZHZ022, repocoder, ReACC}. For example, RAG has been specialized for software engineering tasks such as code generation~\cite{repocoder, ReACC}, which retrieves the similar code from the code base and augments the prompt with the retrieved code for model inference.


==> section/benchmark.tex <==

\subsection{Benchmark \ourbench{}}

\label{sec:dataset}

In this work, we focus on function-level vulnerability detection given it has been widely studied in previous learning-based research~\cite{DBLP:conf/icse/SejfiaDSM24, DBLP:conf/ijcnn/HanifM22, DBLP:conf/icse/SteenhoekGL24, DBLP:conf/uss/MirskyMBYPDML23}. We first revisited widely used function-level vulnerability detection benchmarks and identified two key limitations in existing datasets: (1) the lack of corresponding patched versions for vulnerable code (\eg{} Devign~\cite{DBLP:conf/nips/ZhouLSD019} and Reveal~\cite{DBLP:journals/tse/ChakrabortyKDR22}), and (2) the absence of verified correctness for patched code. For example, although BigVul~\cite{DBLP:conf/msr/FanL0N20} includes patched code, these patches may have been subsequently modified in later CVEs, making their correctness unreliable. 

To this end, we construct a new benchmark \ourbench{}, which specifically targets pairs of vulnerable code and their corresponding patched versions with minor modifications in Linux kernel, as its prevalence and code semantic complexity~\cite{DBLP:conf/apsec/JimenezPT16, li2024llmassistedstaticanalysisdetecting}. 


\parabf{Construction Procedure.}
The benchmark construction process includes two key steps: (i) \textit{Vulnerable and Patched Code Collection}: We extract function-level pairs of vulnerable and patched code, along with descriptions from existing CVEs. (ii) \textit{Patched Code Verification}: To ensure the reliability of the patched code, we verify that it is not subsequently reverted or altered.
The details of the construction process and the final data format are presented in Appendix~\ref{ap:dataset}.

\parabf{Benchmark Statistics.}
As a result, we obtain a new benchmark \ourbench{} of 4314 pairs of vulnerable and patched Linux kernel code functions across 2073 CVEs. In this study, we focus on the top-5 CWEs in our benchmark given the non-trivial costs of model execution and manual analysis. We further randomly divide the benchmark into the training set and the testing set. 
The final training set includes 953 CVEs with 1,462 pairs of vulnerable and patched code functions, while the testing set includes 373 CVEs with 592 pairs. The statistics of each CWE category in our benchmark are shown in Table~\ref{table:benchmark} in Appendix \ref{ap:dataset}.




==> section/construction/knowledge_extraction.tex <==
\subsubsection{Vulnerability Knowledge Extraction}
\label{sec:knowledge_extraction}

In this subsection, we utilize GPT-3.5-turbo to precisely capture vulnerability behavior and solution actions. This task diverges significantly from the process of extracting \csd{}, which merely requires summarizing code purpose and function--a domain where LLMs excel. The capture of vulnerability and solution behaviors imposes significantly higher demands on the LLMs, which involves overcoming two main challenges:

\textbf{Challenge C1: Identifying the root cause of vulnerabilities.} The model needs to fully understand the underlying reasons for the vulnerabilities before summarizing them. Otherwise, it cannot accurately capture the code behavior that truly leads to the vulnerability.

\textbf{Challenge C2: Precise descriptions of Vulnerable Behaviors and Solution Actions.} Once the LLM identifies the root cause of a vulnerability, it is imperative to provide clear and precise descriptions of Vulnerable Behaviors and Solution Actions. Initially, understanding the significance of different elements within vulnerability knowledge poses a challenge. Furthermore, generating knowledge at an appropriate level of granularity is another hurdle. 
Descriptions that are overly generic, such as merely stating the failure to appropriately handle possible asynchronous events leading to a potential use-after-free vulnerability without mentioning the absence of canceling delayed work  (as illustrated in Example 2), or excessively detailed, such as focusing on specific function name, both significantly impact the effectiveness of subsequent RAG-based vulnerability detection.

To address challenge \textbf{C1}, we first explored which input information from commit sources effectively assists the model in understanding the root causes of vulnerabilities. We then leveraged the Chain-of-Thought (CoT) approach to further comprehend the vulnerabilities and extract knowledge from the input.

\textbf{Input:} Through our experimentation, we designated the code snippets in commits(\ie{}vulnerable code snippet and patch code snippet), patch diff, and CVE description as inputs for vulnerability knowledge extraction. This information contributes to the LLM's understanding of the vulnerability. The code snippets in commits provide a before-and-after comparison, while the patch diff highlights the changes made, aiding the LLM in identifying specific vulnerability patterns. Furthermore, the CVE descriptions detail the categories of vulnerabilities and their inherent characteristics, assisting the LLM in deepening its understanding of the vulnerabilities. 

\textbf{Design 1: Chain-of-Thought (CoT).} To encourage the LLMs to ``think step by step" and thus fully understand the root causes of vulnerabilities, we employ a multi-round interaction approach. Given the above input information, we first prompt the model to explain why the modification of the vulnerable code snippet is necessary. Based on the LLM's explanation, we further prompt it to summarize the corresponding vulnerability knowledge. 

To tackle challenge \textbf{C2}, we enhance the quality of generated vulnerability knowledge through few-shot learning and role-playing techniques.

\textbf{Design 2: Few-shot Learning.} To enhance the LLM's comprehension of the significance of different elements within vulnerability knowledge and to summarize vulnerability knowledge at an appropriate level of granularity, we initially manually annotated two instances of vulnerability knowledge as exemplar samples. These samples were presented to the LLM to enable it to fully grasp the desired format and substance of vulnerability knowledge from a limited set of inputs, thereby improving the quality of the summarized vulnerability knowledge. 

\textbf{Design 3: Role-Playing Prompt.} Inspired by previous work\cite{du2023resolving}, we enhance the LLM's ability to understand vulnerabilities by having it role-play as a vulnerability detection expert. This approach is designed to improve the quality of vulnerability knowledge generation further.

The complete iterative process for extracting vulnerability knowledge from the commit information is designed with the following prompt templates: 

\begin{mdframed}
[linecolor=myblue!50,linewidth=2pt,roundcorner=10pt,backgroundcolor=myyellow!20]
\small

\hspace{3.5mm}\textbf{Knowledge Extraction Prompt (Round 1):}  This is a code snippet with a vulnerability [CVE ID]:

[Vulnerable Code Snippet]

The vulnerability is described as follows:[CVE Description]

The correct way to fix it is by [Patch Diff]

The code after modification is as follows:[Patch Code Snippet]

Why is the above modification necessary?

\textbf{Knowledge Extraction Prompt (Round 2):}
I want you to act as a vulnerability detection expert and organize vulnerability knowledge based on the above vulnerability repair information. Please summarize the generalizable specific behavior of the code that leads to the vulnerability and the specific solution to fix it. Format your findings in JSON.
Here are some examples to guide you on the level of detail expected in your extraction:
[Vulnerability  Knowledge Examples]

\end{mdframed}






==> section/data.tex <==
\section{Data Availability}

All the experimental data and source code of our work is available at~\cite{replication_package}.

==> section/discussion.tex <==
\section{Discussion}

\todo{remove this part into threats}

\subsection{Knowledge Representation Design Choice.}


\textbf{Pilot Study. }In our preliminary investigation, our objective was to identify the most effective representation of vulnerability knowledge for enhancing the LLMs' ability to detect vulnerabilities. To this end, we categorized vulnerability knowledge into three distinct types: knowledge based on source code, knowledge derived from static analysis intermediate representations, and knowledge articulated through natural language descriptions. A series of manual trials and analyses were conducted across ten distinct cases to evaluate the comprehensibility and utility of each knowledge type in aiding the LLMs' detection capabilities.

Our findings indicated that the LLM struggled to grasp knowledge derived from historical vulnerable code or results of static analysis, proving these types insufficient for directly assisting LLMs in vulnerability detection. Natural language descriptions concerning different categories of vulnerabilities (e.g., CWE-416, use after free), offered some assistance to the LLMs in detecting corresponding types of vulnerabilities. However, the assistance was limited due to the overly generic nature of the explanations. During our exploration, we discovered that targeted natural language descriptions pinpointing code behaviors that may lead to vulnerabilities directly aid LLMs in detecting corresponding vulnerabilities within code. This observation aligns with findings from prior research\cite{}, confirming that LLMs excel at matching code with its natural language descriptions of behavior.



\subsection{Knowledge Generalizability Across Different CVEs}

In the evaluation phase, we constructed our benchmark test set with CVEs that encompassed multiple instances of vulnerable and patched code pairs, with the intention of ensuring the vulnerability knowledge base contained information pertinent to the code under detection. However, this methodology limited the validation of cases with only a single code pair per CVE. To explore the value of vulnerability knowledge within these cases, we concentrated on the most prevalent vulnerability category, CWE-416, and manually compiled a small-scale dataset comprising 60 code functions (30 positive and 30 negative samples) across 30 unique CVEs, each with only one code pair. For each case in this dataset, we manually verified the presence of relevant vulnerability knowledge extracted from other CVEs in the knowledge base.

During the vulnerability detection process, the use of CVE-specific vulnerability knowledge corresponding to the code snippets under detection was restricted. This limitation required the precise retrieval and utilization of vulnerability knowledge from alternative, related CVEs to capture vulnerable behaviors, thereby facilitating the evaluation of the vulnerability knowledge's generalizability across different CVEs on vulnerability detection. Our approach achieved a recall rate of 0.83 and a precision rate of 0.76 on the dataset, affirming the effectiveness of leveraging vulnerability knowledge from disparate CVEs in enhancing vulnerability detection. 

==> section/evaluation/rq2.tex <==
\subsection{Ablation Studies}

To evaluate the contribution of knowledge-level RAG on enhancing LLMs' performance, we conducted an ablation study comparing \app{} with a variant using code-level RAG. This variant enhances the basic LLM by retrieving similar code snippets from training datasets into the prompts.
The prompt design is detailed in Figure \ref{fig:mov_example} (b) in Appendix \ref{ap:case_rq2}. 


\parabf{Results.}
Table~\ref{table:rq2} shows the comparison between \app{} and the code-level RAG baseline. Overall, \app{} consistently outperforms this variant regarding all metrics, demonstrating the effectiveness of our knowledge-level RAG framework. To further illustrate the superiority of \app{} in both knowledge representation and retrieval strategy, we provide two examples where \app{} successfully detects vulnerabilities while the code-level RAG baseline fails in Appendix \ref{ap:case_rq2}



==> section/evaluation/study_rq.tex <==
\subsubsection{Studied Baselines}
\label{sec:baseline}

We first evaluate the capability of basic LLMs in vulnerability detection across four state-of-the-art LLMs, including two closed-source models: GPT-4-turbo~\cite{gpt4}, Claude Sonnet 3.5~\cite{claude}; and two open-source models: Qwen2.5-Coder-32B-Instruct~\cite{qwen}, DeepSeek-V2-Instruct~\cite{deepseek}. Furthermore, we evaluated advanced LLM-based techniques that employ various optimization strategies to detecting vulnerabilities, including: (1) three approaches leveraging diverse prompt engineering strategies~\cite{DBLP:journals/corr/abs-2308-12697}: role-play strategy, chain-of-thought (CoT) strategy and AST-enhenced strategy; and (2) LLMAO~\cite{DBLP:conf/icse/YangGMH24}, a approach that fine-tunes LLMs for vulnerability detection. 

All advanced LLM-based approaches with prompt strategies are implemented on GPT-4-turbo. For LLMAO, we fine-tune it on our training set for 10 epochs
for adapting the techniques to our benchmark. As LLMAO is a line-level vulnerability detection technique, we adapt it to the function level by regarding the function that has any line with higher-than-0.5 suspiciousness scores as vulnerable. For more detailed descriptions of these advanced baselines, we provide them in Appendix~\ref{ap:baseline}.



\subsubsection{Metrics}
We evaluate the capability in distinguishing a pair of vulnerable code and patched code by the following three metrics. 
(1) \textbf{\pairacc{}}, which calculates among all pairs, the ratio of pairs whose vulnerable and patched code are both correctly identified;
(2) \textbf{\vulrate{}}, which calculates among the pairs whose vulnerable is correctly identified, the ratio of pairs whose patched code is incorrectly identified as vulnerable; 
(2) \textbf{\patchrate{}}, which calculates among the pairs whose patched is correctly identified, the ratio of pairs whose vulnerable code is incorrectly identified as benign. 

Additionally, we also use six commonly-used metrics in vulnerability detection tasks, \ie FN, FP, accuracy, precision, recall, and F1. FN is the ratio of false negatives; FP is the ratio of false positives; accuracy is the proportion of correctly detected instances; precision is the proportion of true positive predictions among all positive predictions; recall is the proportion of true positive predictions among all instances; and F1-score is the harmonic mean of the precision and recall, which balances both values.



\subsubsection{Results}
 

\input{table/study_result}



==> table/all_result.tex <==



\begin{table}[htb]
    \centering
    \caption{Effectiveness in CWE-119} \label{table:119}
        \begin{adjustbox}{width=0.6\linewidth}
            \begin{tabular}{c|c|c|c|c}
            \hline
            \textbf{Tech.} & \textbf{LLM} & \textbf{Pair Acc.} & \textbf{Bal. Recall} & \textbf{Bal. Pre.}  \\ \hline
    
            \multirow{4}{*}{Basic LLM}
            & GPT-4o & 0.05  & 0.50 & 0.50  \\
            & Claude & 0.09 & 0.51 & 0.51\\
            & Qwen & 0.02  & 0.51 & 0.52 \\
            & DeepSeek & 0.13 & 0.49 & 0.48 \\\hline 
            
            \multirow{4}{*}{CoT-1}
            & GPT-4o & 0.18  & 0.50 & 0.50  \\
            & Claude & 0.09 & 0.47 & 0.46\\
            & Qwen & 0.07  & 0.49 & 0.48 \\
            & DeepSeek & 0.14  & 0.51 & 0.52 \\\hline 
            
            \multirow{4}{*}{CoT-2}
            & GPT-4o & 0.16  & 0.50 & 0.50 \\
            & Claude & 0.07  & 0.45 & 0.45  \\
            & Qwen & 0.10 & 0.47 & 0.46 \\
            & DeepSeek & 0.07 & 0.51 & 0.53\\\hline 
    
            \multirow{4}{*}{\tabincell{c}{CWE\\Enhanced}}
            & GPT-4o & 0.18 & 0.53 & 0.53 \\
            & Claude & 0.09  & 0.51 & 0.52  \\
            & Qwen & 0.02  & 0.51 & 0.53 \\
            & DeepSeek & 0.11 & 0.50 & 0.50 \\ \hline
    
            \multirow{4}{*}{Code RAG
            }& GPT-4o & 0.05  & 0.52 & 0.63 \\
            & Claude & 0.09  & 0.53 & 0.54  \\
            & Qwen & 0.10  & 0.55 & 0.57 \\
            & DeepSeek & 0.0  & 0.50 & 0.25\\\hline

            \multirow{2}{*}{LLMAO
            } & Qwen & 0.03 & 0.50 & 0.50\\
            & DeepSeek-R1-7b & 0.03 & 0.50 & 0.50\\ \hline     
            
            \multirow{4}{*}{\app{}
            }& GPT-4o & 0.26 & 0.56 & 0.59\\
            & Claude & 0.20  & 0.57 & 0.58 \\
            & Qwen & 0.23  & 0.60 & 0.66 \\
            & DeepSeek & 0.30 & 0.63 & 0.65 \\\hline 
            \end{tabular}
    \end{adjustbox}
        
\end{table}
\begin{table}
    \centering
    \caption{Effectiveness in CWE-476} \label{table:all_result}
        \begin{adjustbox}{width=0.6\linewidth}
            \begin{tabular}{c|c|c|c|c}
            \hline
            \textbf{Tech.} & \textbf{LLM} & \textbf{Pair Acc.} & \textbf{Bal. Recall} & \textbf{Bal. Pre.}  \\ \hline
    
            \multirow{4}{*}{Basic LLM}
            & GPT-4o & 0.03  & 0.49 & 0.48  \\
            & Claude & 0.06 & 0.51 & 0.52\\
            & Qwen & 0.04  & 0.50 & 0.50 \\
            & DeepSeek & 0.23 & 0.56 & 0.60 \\\hline 
            
            \multirow{4}{*}{CoT-1}
            & GPT-4o & 0.17  & 0.49 & 0.49  \\
            & Claude & 0.15 & 0.56 & 0.56\\
            & Qwen & 0.06  & 0.46 & 0.42 \\
            & DeepSeek & 0.14  & 0.50 & 0.50 \\\hline 
            
            \multirow{4}{*}{CoT-2}
            & GPT-4o & 0.21  & 0.54 & 0.54 \\
            & Claude & 0.21  & 0.56 & 0.56  \\
            & Qwen & 0.18 & 0.49 & 0.49 \\
            & DeepSeek & 0.17 & 0.53 & 0.54\\\hline 
    
            \multirow{4}{*}{\tabincell{c}{CWE\\Enhanced}}
            & GPT-4o & 0.14 & 0.49 & 0.49 \\
            & Claude & 0.18  & 0.52 & 0.52  \\
            & Qwen & 0.04  & 0.51 & 0.53 \\
            & DeepSeek & 0.25 & 0.57 & 0.57 \\ \hline
    
            \multirow{4}{*}{Code RAG
            }& GPT-4o & 0.07  & 0.52 & 0.61 \\
            & Claude & 0.17  & 0.54 & 0.56  \\
            & Qwen & 0.07  & 0.54 & 0.65 \\
            & DeepSeek & 0.03  & 0.51 & 0.75\\\hline

            \multirow{2}{*}{LLMAO
            } & Qwen & 0.02 & 0.48 & 0.47\\
            & DeepSeek-R1-7b & 0.04 & 0.51 & 0.51\\             \hline 
            
            \multirow{4}{*}{\app{}
            }& GPT-4o & 0.31 & 0.56 & 0.65\\
            & Claude & 0.21  & 0.58 & 0.59 \\
            & Qwen & 0.24  & 0.57 & 0.58 \\
            & DeepSeek & 0.26 & 0.61 & 0.61 \\\hline 
            \end{tabular}
    \end{adjustbox}
        
\end{table}

\begin{table}
    \centering
    \caption{Effectiveness in CWE-787} \label{table:all_result}
        \begin{adjustbox}{width=0.6\linewidth}
            \begin{tabular}{c|c|c|c|c}
            \hline
            \textbf{Tech.} & \textbf{LLM} & \textbf{Pair Acc.} & \textbf{Bal. Recall} & \textbf{Bal. Pre.}  \\ \hline
    
            \multirow{4}{*}{Basic LLM}
            & GPT-4o & 0.11  & 0.51 & 0.52  \\
            & Claude & 0.02 & 0.49 & 0.49\\
            & Qwen & 0.09  & 0.53 & 0.54 \\
            & DeepSeek & 0.17  & 0.54 & 0.56 \\\hline 
            
            \multirow{4}{*}{CoT-1}
            & GPT-4o & 0.23  & 0.55 & 0.55  \\
            & Claude & 0.05 & 0.46 & 0.46\\
            & Qwen & 0.15  & 0.50 & 0.50 \\
            & DeepSeek & 0.10  & 0.51 & 0.52 \\\hline 
            
            \multirow{4}{*}{CoT-2}
            & GPT-4o & 0.23  & 0.55 & 0.58 \\
            & Claude & 0.09  & 0.52 & 0.53  \\
            & Qwen & 0.19 & 0.52 & 0.53 \\
            & DeepSeek & 0.17 & 0.57 & 0.63\\\hline 
    
            \multirow{4}{*}{\tabincell{c}{CWE\\Enhanced}}
            & GPT-4o & 0.08 & 0.50 & 0.50 \\
            & Claude & 0.13  & 0.55 & 0.65  \\
            & Qwen & 0.04  & 0.51 & 0.54 \\
            & DeepSeek & 0.15 & 0.54 & 0.55 \\ \hline
    
            \multirow{4}{*}{Code RAG
            }& GPT-4o & 0.06  & 0.53 & 0.61 \\
            & Claude & 0.11  & 0.50 & 0.50  \\
            & Qwen & 0.09  & 0.50 & 0.50 \\
            & DeepSeek & 0.0  & 0.50 & 0.25\\\hline

            \multirow{2}{*}{LLMAO
            } & Qwen & 0.06 & 0.51 & 0.52\\
            & DeepSeek-R1-7b & 0.06 & 0.51 & 0.52\\ \hline
            
            \multirow{4}{*}{\app{}
            }& GPT-4o & 0.28 & 0.70 & 0.57\\
            & Claude & 0.19  & 0.57 & 0.59 \\
            & Qwen & 0.21  & 0.57 & 0.58 \\
            & DeepSeek & 0.32 & 0.60 & 0.60 \\\hline 
            \end{tabular}
    \end{adjustbox}
        
\end{table}

\begin{table}
    \centering
    \caption{Effectiveness in CWE-362} \label{table:all_result}
        \begin{adjustbox}{width=0.6\linewidth}
            \begin{tabular}{c|c|c|c|c}
            \hline
            \textbf{Tech.} & \textbf{LLM} & \textbf{Pair Acc.} & \textbf{Bal. Recall} & \textbf{Bal. Pre.}  \\ \hline
    
            \multirow{4}{*}{Basic LLM}
            & GPT-4o & 0.05  & 0.46 & 0.45  \\
            & Claude & 0.07 & 0.53 & 0.53\\
            & Qwen & 0.07  & 0.51 & 0.51 \\
            & DeepSeek & 0.10  & 0.50 & 0.51 \\\hline 
            
            \multirow{4}{*}{CoT-1}
            & GPT-4o & 0.17  & 0.46 & 0.46  \\
            & Claude & 0.12 & 0.49 & 0.49\\
            & Qwen & 0.07  & 0.48 & 0.46 \\
            & DeepSeek & 0.17  & 0.53 & 0.54 \\\hline 
            
            \multirow{4}{*}{CoT-2}
            & GPT-4o & 0.16  & 0.46 & 0.45 \\
            & Claude & 0.11  & 0.50 & 0.50  \\
            & Qwen & 0.16 & 0.54 & 0.54 \\
            & DeepSeek & 0.11 & 0.48 & 0.47\\\hline 
    
            \multirow{4}{*}{\tabincell{c}{CWE\\Enhanced}}
            & GPT-4o & 0.19 & 0.53 & 0.55 \\
            & Claude & 0.16  & 0.54 & 0.55  \\
            & Qwen & 0.10  & 0.52 & 0.53 \\
            & DeepSeek & 0.22 & 0.56 & 0.56 \\ \hline
    
            \multirow{4}{*}{Code RAG
            }& GPT-4o & 0.02  & 0.51 & 0.54 \\
            & Claude & 0.10  & 0.52 & 0.54  \\
            & Qwen & 0.07  & 0.52 & 0.53 \\
            & DeepSeek & 0.0  & 0.49 & 0.25\\\hline

            \multirow{2}{*}{LLMAO
            } & Qwen & 0.06 & 0.51 & 0.52\\
            & DeepSeek-R1-7b & 0.06 & 0.51 & 0.52\\ \hline 
            
            \multirow{4}{*}{\app{}
            }& GPT-4o & 0.31 & 0.56 & 0.61\\
            & Claude & 0.25  & 0.60 & 0.61 \\
            & Qwen & 0.22  & 0.57 & 0.57 \\
            & DeepSeek & 0.25 & 0.60 & 0.62  \\\hline 
            \end{tabular}
    \end{adjustbox}
        
\end{table}



\begin{table}
    \centering
    \caption{Effectiveness in CWE-416} \label{table:416}
        \begin{adjustbox}{width=0.6\linewidth}
            \begin{tabular}{c|c|c|c|c}
            \hline
            \textbf{Tech.} & \textbf{LLM} & \textbf{Pair Acc.} & \textbf{Bal. Recall} & \textbf{Bal. Pre.}  \\ \hline
    
            \multirow{4}{*}{Basic LLM}
            & GPT-4o & 0.13  & 0.49 & 0.49  \\
            & Claude & 0.14 & 0.49 & 0.49\\
            & Qwen & 0.13  & 0.53 & 0.43 \\
            & DeepSeek & 0.10  & 0.50 & 0.50 \\\hline 
            
            \multirow{4}{*}{CoT-1}
            & GPT-4o & 0.22  & 0.53 & 0.53  \\
            & Claude & 0.13 & 0.51 & 0.51\\
            & Qwen & 0.08  & 0.50 & 0.50 \\
            & DeepSeek & 0.17  & 0.52 & 0.52 \\\hline 
            
            \multirow{4}{*}{CoT-2}
            & GPT-4o & 0.16 & 0.47 & 0.47 \\
            & Claude & 0.10  & 0.50 & 0.50  \\
            & Qwen & 0.19 & 0.52 & 0.52 \\
            & DeepSeek & 0.14 & 0.52 & 0.53 \\\hline 
    
            \multirow{4}{*}{\tabincell{c}{CWE\\Enhanced}}
            & GPT-4o & 0.07 & 0.50 & 0.48 \\
            & Claude & 0.05  & 0.49 & 0.46  \\
            & Qwen & 0.0  & 0.48 & 0.33 \\
            & DeepSeek & 0.11 & 0.52 & 0.54 \\ \hline
    
            \multirow{4}{*}{Code RAG
            }& GPT-4o & 0.04  & 0.50 & 0.51 \\
            & Claude & 0.10  & 0.51 & 0.52  \\
            & Qwen & 0.12  & 0.55 & 0.62 \\
            & DeepSeek & 0.01  & 0.50 & 0.50\\\hline

            \multirow{2}{*}{LLMAO
            } & Qwen & 0.07 & 0.52 & 0.52\\
            & DeepSeek-R1-7b & 0.01  & 0.50 & 0.50\\ \hline 
            
            \multirow{4}{*}{\app{}
            }& GPT-4o & 0.28 & 0.60 & 0.57\\
            & Claude & 0.32  & 0.63 & 0.64 \\
            & Qwen & 0.24  & 0.58 & 0.60 \\
            & DeepSeek & 0.29 & 0.58 & 0.59 \\\hline 
            \end{tabular}
    \end{adjustbox}
        
\end{table}



==> table/cwe_statistics.tex <==
\begin{table*}[htb]
	%\scriptsize
    \centering
	%\vspace{-5mm}
    \caption{The Statistics of the 10 Most Frequent CWEs}	 
    \label{table:cwe}
    \footnotesize
    \begin{adjustbox}{width=1\textwidth}
    \begin{tabular}{|p{4cm}<{\centering}|p{1cm}<{\centering}|p{1.2cm}<{\centering}|p{10cm}<{\raggedright}|} \hline
	
    \textbf{CWE ID \& Name}  & \textbf{CVE Num.}  & \textbf{Fun. Pair Num.}  & \textbf{CWE Description} \\  \hline
    CWE-416: Use After Free & 341 & 856 & Referencing memory after it has been freed can cause a program to crash, use unexpected values, or execute code. \\  \hline
    CWE-476: NULL Pointer Dereference & 196 & 353 & A NULL pointer dereference occurs when the application dereferences a pointer that it expects to be valid, but is NULL, typically causing a crash or exit. \\  \hline
    CWE-362: Concurrent Execution using Shared Resource with Improper Synchronization  & 170 & 402 & The product contains a code sequence that can run concurrently with other code, and the code sequence requires temporary, exclusive access to a shared resource, but a timing window exists in which the shared resource can be modified by another code sequence that is operating concurrently. \\  \hline
    CWE-119: Improper Restriction of Operations within the Bounds of a Memory Buffer & 130 & 217 & The product performs operations on a memory buffer, but it can read from or write to a memory location that is outside of the intended boundary of the buffer. \\  \hline
    CWE-787: Out-of-bounds Write & 124 & 235 & The product writes data past the end, or before the beginning, of the intended buffer. \\  \hline
    CWE-200: Exposure of Sensitive Information to an Unauthorized Actor & 116 & 208 & The product exposes sensitive information to an actor that is not explicitly authorized to have access to that information. \\  \hline
    CWE-125: Out-of-bounds Read & 106 & 177 & The product reads data past the end, or before the beginning, of the intended buffer. \\  \hline
    CWE-20: Improper Input Validation & 96 & 283 & The product receives input or data, but it does not validate or incorrectly validates that the input has the properties that are required to process the data safely and correctly. \\  \hline
    CWE-401: Missing Release of Memory after Effective Lifetime & 94 & 128 & The product does not sufficiently track and release allocated memory after it has been used, which slowly consumes remaining memory. \\  \hline
    CWE-190: Integer Overflow or Wraparound & 46 & 64 & The product performs a calculation that can produce an integer overflow or wraparound, when the logic assumes that the resulting value will always be larger than the original value. This can introduce other weaknesses when the calculation is used for resource management or execution control. \\  \hline
    \end{tabular}
    \end{adjustbox}
    % \vspace{-1mm}
\end{table*}

==> table/definition.tex <==
\begin{table*}[htb]
	%\scriptsize
    \centering
	%\vspace{-5mm}
    \caption{Definitions of Elements in Vulnerability Knowledge Representation}	 
    \label{table:def}
    \footnotesize
    \begin{adjustbox}{width=1\textwidth}
    \begin{tabular}{|p{2.5cm}<{\centering}|p{2.5cm}<{\centering}|p{9cm}<{\raggedright}|} \hline
	
    \textbf{Element Name} & \textbf{Dimension}  & \textbf{Definition} \\  \hline
    Purpose  &  Functional Semantics &  Describes the intended goal or function that the code snippet aims to fulfill within the broader framework of the system's architecture.
    \\  \hline
    Function & Functional Semantics &  Describes the detailed operations or sequence of actions executed by the code, providing insight into its operational mechanics. 
    \\ \hline 
    Precondition  & Vulnerability Behavior & Describes the initial conditions or scenarios that may predispose the code to potential vulnerabilities.  
    \\ \hline  
    Trigger Condition  & Vulnerability Behavior &  Describes the specific event or action that activates or exploits an existing vulnerability, often dependent on external stimuli or specific states that trigger the vulnerability.
    \\ \hline 
    Vulnerability Description & Vulnerability Behavior &  Describes the precise behaviors (\eg{} the erroneous logic, design flaws, or implementation mistakes) within the code that directly lead to a vulnerability.
    \\ \hline 
    Solution Description & Solution Action &  Describes the devised strategy to  resolve the identified vulnerability. 
    \\ \hline 
    Solution Implementation & Solution Action & Describes the practical application details of the solution, including (1) Action: a succinct summary of the solution action taken. (2) Code: the code modifications associated with the solution action. (3) Rationale: The underlying reasoning for the chosen solution approach.
    \\ \hline
    \end{tabular}
    \end{adjustbox}
    % \vspace{-1mm}
\end{table*}

==> table/exist_benchmark.tex <==
\begin{table*}[htb]
	%\scriptsize
    \centering
	%\vspace{-5mm}
    \caption{Existing Benchmarks for Vulnerability Detection.
    ``Positive Number/Ratio'' is the number/portion of vulnerable samples,  ``\#CVE'' is the number of CVEs, ``Positive LOC''/``Negative LOC'' is the average lines numbers of vulnerable/non-vulnerable code, ``Patched Code Included'' means whether the patched code of the vulnerability is included, ``Patched Code Verified'' means whether patched code is verified as correct, and ``Data Sources'' indicates whether the datasets include Linux data, ``Mixed Linux'' represents sources that include both Linux and other projects.}
    % \todo{make the table smaller}}	 
    \label{table:exist_benchmark}
    \footnotesize
    \begin{adjustbox}{width=0.95\textwidth}
        \begin{tabular}{@{} m{1.5cm}<{\centering}|m{1cm}<{\centering}|m{2.5cm}<{\centering}|m{1.5cm}<{\centering}|m{1cm}<{\centering}|m{1cm}<{\centering}|m{1.5cm}<{\centering}|m{1.5cm}<{\centering} @{}|m{2cm}<{\centering}}
            \hline
            \textbf{Benchmark} & \textbf{Time} & \textbf{Positive Number/Ratio}  & \textbf{\#CVE} & \textbf{Positive LOC} & \textbf{Negative LOC} & \textbf{Patched Code Included} & \textbf{Patched Code Verified} & \textbf{Data Source} \\ \hline
            % DiverseVul & 2023 & Security Issues & 18945 & 5.73 \% & / & 114.71 & 39.26 & Y & N \\ \hline
            BigVul & 2020 & 10,900(5.78\%) & 3,285 & 73.47 & 23.83 & N & / & Mixed Linux \\ \hline
            Devign & 2019  & 12,460 (45.61\%) & / & 54.50 & 49.53 & N & / & No Linux\\ \hline
            ReVeal & 2020  & 2,240 ( 9.85\%) & / & 67.73 & 28.69 & Y & N & No Linux\\ \hline \hline 
             \ourbench{} & 2024 & 1,923 (50.00\%) & 896 & 68.58 & 70.25 & Y & Y & Only Linux  \\ \hline
        \end{tabular}
        \end{adjustbox}
\end{table*}


==> table/rq2_result.tex <==


\begin{table}[htb]
	%\scriptsize
    \centering
    %\vspace{-1mm}
    \caption{Effectiveness of \app{} and GPT-4-based techniques (RQ1\& RQ2)}	 
    \label{table:rq2}
    \footnotesize
    \begin{adjustbox}{width=0.9\linewidth}
        \begin{tabular}{c|c|c|c|c|c|c|c}
        \hline
        \textbf{Tech.} & \textbf{FN} & \textbf{FP} & \textbf{Acc.} & \textbf{Pair Acc.} & \textbf{Precis.} & \textbf{Recall} & \textbf{F1} \\ \hline
        Basic Prompt & 49.0 \% & 1.5 \% & 0.5 & 0.01 & 0.4 & 0.02 & 0.04 \\
        Role-Play Enhanced Prompt & 41.1 \% & 8.9 \% & 0.49 & 0.05 & 0.49 & 0.21 & 0.3 \\
        CoT Enhanced Prompt & 38.5 \% & 7.0 \% & 0.55 & 0.13 & \textbf{0.61} & 0.23 & 0.34 \\
        AST Enhanced Prompt & 41.9 \% & 7.6 \% & 0.51 & 0.05 & 0.52 & 0.16 & 0.25 \\
        Code-based RAG & 38.3 \% & 11.5 \% & 0.5 & 0.01 & 0.51 & 0.23 & 0.32 \\
        VUL-RAG & 19.4 \% & 19.8 \% & \textbf{0.61} & \textbf{0.21} &\textbf{0.61} & \textbf{0.61} & \textbf{0.61} \\ \hline
        \end{tabular}
        \end{adjustbox}
\end{table}

==> table/study_result.tex <==


\begin{table}[htb]
    \centering
    \caption{Evaluation of Basic LLMs}\label{table:rq1}
    \footnotesize
    \begin{adjustbox}{width=0.98\linewidth}
        \begin{tabular}{c|c|c|c}
        \hline
        \textbf{LLMs} & \textbf{Pair Acc.} & \textbf{Bal. Recall} & \textbf{Bal. Pre.} \\ \hline
        GPT-4 & 0.05  & 0.50 & 0.50\\
        Claude & 0.05  & 0.49 & 0.49\\
        Qwen & 0.04  & 0.49 & 0.49\\
        DeepSeek & 0.06 & 0.48 & 0.48\\
        \hline
        \end{tabular}
    \end{adjustbox}
\end{table}


\begin{table}[htb]
    \centering
    \caption{Impacts of Enhancement Techniques}\label{table:rq2}
    \footnotesize
    \begin{adjustbox}{width=1\linewidth}
        \begin{tabular}{c|c|c|c|c}
        \hline
        \textbf{Tech.} & \textbf{LLM} & \textbf{Pair Acc.} & \textbf{Bal. Recall} & \textbf{Bal. Pre.}\\ \hline

        \multirow{4}{*}{CoT-1}& GPT-4 & 0.14  & 0.49 & 0.49  \\
        & Claude & 0.14 & 0.51 & 0.51\\
        & Qwen & 0.02  & 0.51 & 0.55 \\
        & DeepSeek & 0.09  & 0.50 & 0.50 \\\hline 
        
        \multirow{4}{*}{CoT-2}& GPT-4 & 0.10  & 0.51 & 0.52 \\
        & Claude & 0.14  & 0.53 & 0.53  \\
        & Qwen & 0.16 & 0.52 & 0.52 \\
        & DeepSeek & 0.12 & 0.51 & 0.51\\\hline 

        \multirow{4}{*}{\tabincell{c}{CWE\\Enhanced}}& GPT-4 & 0.03 & 0.50 & 0.50 \\
        & Claude & 0.04  & 0.50 & 0.51  \\
        & Qwen & 0.03  & 0.50 & 0.49 \\
        & DeepSeek & 0.01 & 0.50 & 0.42 \\ \hline

        \end{tabular}
    \end{adjustbox}
\end{table}



